An Accelerated Algorithm for Stochastic Bilevel Optimization under Unbounded Smoothness

This paper investigates a class of stochastic bilevel optimization problems where the upper-level function is nonconvex with potentially unbounded smoothness and the lower-level problem is strongly convex. These problems have significant applications in sequential data learning, such as text classification using recurrent neural networks. The unbounded smoothness is characterized by the smoothness constant of the upper-level function scaling linearly with the gradient norm, lacking a uniform upper bound. Existing state-of-the-art algorithms require $\widetilde{O}(1/\epsilon^4)$ oracle calls of stochastic gradient or Hessian/Jacobian-vector product to find an $\epsilon$-stationary point. However, it remains unclear if we can further improve the convergence rate when the assumptions for the function in the population level also hold for each random realization almost surely. To address this issue, we propose a new Accelerated Bilevel Optimization algorithm named AccBO. The algorithm updates the upper-level variable by normalized stochastic gradient descent with recursive momentum and the lower-level variable by the stochastic Nesterov accelerated gradient descent algorithm with averaging. We prove that our algorithm achieves an oracle complexity of $\widetilde{O}(1/\epsilon^3)$ to find an $\epsilon$-stationary point, when the lower-level stochastic gradient's variance is $O(\epsilon)$. Our proof relies on a novel lemma characterizing the dynamics of stochastic Nesterov accelerated gradient descent algorithm under distribution drift with high probability for the lower-level variable, which is of independent interest and also plays a crucial role in analyzing the hypergradient estimation error over time. Experimental results on various tasks confirm that our proposed algorithm achieves the predicted theoretical acceleration and significantly outperforms baselines in bilevel optimization.

==> nesterov_single_level.tex <==
For convenience, we will restate a few concepts included in \Cref{sec:nesterov} here. We consider the sequences of stochastic optimization problems 
\begin{equation} \label{eq:obj-time-drift}
    \min_{w\in\R^d} \phi_t(w) 
\end{equation}
indexed by time $t\in\mathbb{N}$. We denote the minimizer and the minimal value of $\phi_t$ as $w_t^*$ and $\phi_t^*$, and we define the \textit{minimizer drift} at time $t$ to be $\Delta_t\coloneqq \|w_t^*-w_{t+1}^*\|$. With a slight abuse of notation, we consider the SNAG algorithm applied to the sequence $\{\phi_t\}_{t=1}^{T}$, where $T$ is the total number of iterations:
\begin{equation}
\label{eq:NAG-single}
\begin{aligned}
    z_t &= w_t + \gamma(w_t-w_{t-1})  \\
    w_{t+1} &= w_t + \gamma(w_t-w_{t-1}) - \alpha g_t, 
\end{aligned}
\end{equation}
where $g_t=\nabla \phi_t(z_t;\xi_t)$ is the stochastic gradient evaluated at $z_t$ with random sample $\xi_t$. Define $\varepsilon_t=g_t-\nabla \phi_t(z_t)$ as the stochastic gradient noise at $t$-th iteration. Define $\mathcal{H}_t=\sigma(\xi_1,\ldots,\xi_{t-1})$ as the filtration, which is the $\sigma$-algebra generated by all random variables until $t$-th iteration. We will make the following standard assumption, as illustrated below~\footnote{Note that \cref{ass:sc-smooth-single-level,ass:noise-drift-single-level} are more concrete than that in \Cref{sec:nesterov}.}.

\begin{assumption} \label{ass:sc-smooth-single-level}
The sequences of time-varying functions satisfy that, each function $\phi_t : \R^d \rightarrow \R$ is $\mu$-strongly convex and $L$-smooth for some constants $\mu,L > 0$.
\end{assumption}

\begin{assumption}[Sub-Gaussian drift and noise] \label{ass:noise-drift-single-level}
There exists constants $\Delta,\sigma>0$ such that the following holds for all $t\geq0$:
\begin{enumerate}[(i)]
    \item (\textbf{Drift}) The drift $\Delta_t^2$ is sub-exponential conditioned on $\gH_t$ with parameter $\Delta^2$:
    \begin{equation*}
        \E\left[\exp(\lambda\Delta_t^2) \mid \gH_t\right] \leq \exp(\lambda\Delta^2)
        \quad\text{for all}\quad
        0\leq \lambda\leq \Delta^{-2}.
    \end{equation*}
    \item (\textbf{Noise}) The noise $\varepsilon_t$ is norm sub-Gaussian conditioned on $\gH_t$ with parameter $\sigma/2$:
    \begin{equation*}
        \pr\left\{\|\varepsilon_t\|\geq \varrho \mid \gH_t \right\} \leq 2\exp(-2\varrho^2/\sigma^2)
        \quad\text{for all}\quad
        \varrho > 0.
    \end{equation*}
\end{enumerate}
\end{assumption}

The following lemma characterize the one-step improvement for stochastic Nesterov accelerated gradient method. Although part of our analysis is similar to \cite{chen2023convergence,aybat2020robust}, our final goal is quite different: we aim to derive a careful formulation (see \eqref{eq:one-step-single-level}) such that we can apply \Cref{lm:recursive-control} to recursively control the moment generating function of $V_t$ with distributional drift, thus leading to a high probability bound for $V_t$ at \textit{anytime} (see \Cref{lm:dist-track-single-level}), while \cite{chen2023convergence,aybat2020robust} only show the convergence in expectation without distributional drift. 

\begin{lemma}[Distance recursion, with drift] \label{lm:distance-recursion-single-level}
Suppose that \cref{ass:sc-smooth-single-level,ass:noise-drift-single-level} hold. Let $\{w_t\}$ be the iterates produced by update rule \eqref{eq:NAG-single} with constant learning rate $\alpha\leq 1/2L$ and set constants $\gamma, \rho>0$, and matrix $\rmP\in\R^{2d\times 2d}$ as
\begin{equation} \label{eq:gamma-rhp-P}
    \gamma = \frac{1-\sqrt{\mu\alpha}}{1+\sqrt{\mu\alpha}},
    \quad
    \rho^2 = 1-\sqrt{\mu\alpha},
    \quad
    \rmP = \frac{1}{2\alpha}
    \begin{bmatrix}
        1 & \sqrt{\mu\alpha}-1 \\
        \sqrt{\mu\alpha}-1 & (1-\sqrt{\mu\alpha})^2
    \end{bmatrix} \otimes \rmI_d.
\end{equation}
Define $\theta_t = [(w_t-w_t^*)^{\top}, (w_{t-1}-w_t^*)^{\top}]^{\top} \in \R^{2d}$, also define the potential function and $u_{t,1}, u_{t,2}$ as 
\begin{equation} \label{eq:potential-V}
    V_t = \theta_t^{\top}\rmP\theta_t + \phi_t(w_t) - \phi_t(w_t^*), 
    \quad\quad
    u_{t,1} = \frac{w_t-w_t^*}{\|w_t-w_t^*\|},
    \quad\quad
    u_{t,2} = \frac{z_t-w_t}{\|z_t-w_t\|}.
\end{equation}
Then for all $t\geq0$, it holds that
\begin{equation} \label{eq:all-d}
    \begin{aligned}
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}
        &+ \phi_t(w_{t+1}) - \phi_t(w_t^*) \\
        &\leq \rho^2V_t - \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2.
    \end{aligned}
\end{equation}
Specifically, if $\phi_t(w) \coloneqq \frac{\mu}{2}\|w-w_t^*\|^2$, then we have
\begin{equation} \label{eq:one-step-single-level}
    \begin{aligned}
        V_{t+1}
        &\leq \left(1-\frac{\sqrt{\mu\alpha}}{2}\right)V_t + \left(1+\frac{\sqrt{\mu\alpha}}{4}\right) 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] + \frac{20\mu\Delta_t^2}{\sqrt{\mu\alpha}}.
    \end{aligned}
\end{equation}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:distance-recursion-single-level}]
We first apply \Cref{lm:P-norm-young} with 
\begin{equation*}
    v_1+v_2 = \theta_{t+1} = 
    \begin{bmatrix}
        w_{t+1}-w_{t+1}^* \\
        w_t - w_{t+1}^*
    \end{bmatrix},
    \quad
    v_1 = 
    \begin{bmatrix}
        w_{t+1} - w_t^* \\
        w_t - w_t^* 
    \end{bmatrix},
    \quad
    v_2 = 
    \begin{bmatrix}
        w_t^* - w_{t+1}^* \\
        w_t^* - w_{t+1}^*
    \end{bmatrix},
    \quad
    \rmQ = \rmP
\end{equation*}
to obtain
\begin{small}
\begin{equation*}
    \begin{aligned}
        &V_{t+1} 
        = \theta_{t+1}^{\top}\rmP\theta_{t+1} + \phi_{t+1}(w_{t+1}) - \phi_{t+1}(w_{t+1}^*) \\
        &\leq \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}
        + 
        \left(1+\frac{4}{\sqrt{\mu\alpha}}\right)
        \begin{bmatrix}
            w_t^* - w_{t+1}^* \\
            w_t^* - w_{t+1}^*
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_t^* - w_{t+1}^* \\
            w_t^* - w_{t+1}^*
        \end{bmatrix}
        + \phi_{t+1}(w_{t+1}) - \phi_{t+1}(w_{t+1}^*) \\
        &= 
        \underbrace{\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\left\{
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix} 
        + \phi_t(w_{t+1}) - \phi_t(w_t^*)
        \right\}}_{(A)} \\
        &\quad+ \underbrace{\phi_{t+1}(w_{t+1}) - \phi_{t+1}(w_{t+1}^*) - \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)(\phi_t(w_{t+1}) - \phi_t(w_t^*))}_{(B)} 
        + \underbrace{\left(1+\frac{4}{\sqrt{\mu\alpha}}\right)
        \begin{bmatrix}
            w_t^* - w_{t+1}^* \\
            w_t^* - w_{t+1}^*
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_t^* - w_{t+1}^* \\
            w_t^* - w_{t+1}^*
        \end{bmatrix}}_{(C)}.
    \end{aligned}
\end{equation*}
\end{small}%
Now we bound terms $(A)$, $(B)$ and $(C)$ individually. 

\paragraph{Bounding $(A)$.}
Let us define vector $\omega_t\in\R^{d}$ and matrices $\rmA\in\R^{2d\times 2d}, \rmB\in\R^{2d\times d}$ as 
% $\rmA,\rmB\in\R^{2d\times 2d}$ as 
\begin{equation*}
    % \omega_t = 
    % \begin{bmatrix}
    %     \nabla \phi_t(z_t) \\
    %     \varepsilon_t
    % \end{bmatrix},
    \omega_t = \nabla \phi_t(z_t),
    \quad
    \rmA = 
    \begin{bmatrix}
        1+\gamma & -\gamma \\
        1 & 0
    \end{bmatrix} \otimes \rmI_d,
    \quad
    % \rmB = 
    % \begin{bmatrix}
    %     -\alpha & -\alpha \\
    %     0 & 0
    % \end{bmatrix} \otimes \rmI_d.
    \rmB = 
    \begin{bmatrix}
        -\alpha \\
        0 
    \end{bmatrix} \otimes \rmI_d.
\end{equation*}
By \eqref{eq:NAG-single} we have 
$[(w_{t+1} - w_t^*)^{\top}, (w_t - w_t^*)^{\top}]^{\top} = \rmA\theta_t + \rmB(\omega_t + \varepsilon_t)$. 
% $[(w_{t+1} - w_t^*)^{\top}, (w_t - w_t^*)^{\top}]^{\top} = \rmA\theta_t + \rmB\omega_t$. 
% \begin{equation*}
%     \begin{aligned}
%         \begin{bmatrix}
%             w_{t+1} - w_t^* \\
%             w_t - w_t^* 
%         \end{bmatrix}
%         = \rmA\theta_t + \rmB\omega_t.
%     \end{aligned}
% \end{equation*}
Since $\phi_t$ is $\mu$-strongly convex, then
\begin{equation} \label{eq:phi-t-SC}
    \phi_t(w_t) - \phi_t(z_t) \geq \langle \nabla\phi_t(z_t), w_t-z_t \rangle + \frac{\mu}{2}\|w_t-z_t\|^2.
\end{equation}
By $L$-smoothness of $\phi_t$ and the fact that $w_{t+1} = z_t - \alpha g_t$, we have
\begin{equation} \label{eq:phi-t-smooth}
    \begin{aligned}
        \phi_t(z_t) &- \phi_t(w_{t+1})
        \geq \langle \nabla\phi_t(z_t), z_t-w_{t+1} \rangle - \frac{L}{2}\|w_{t+1}-z_t\|^2 \\
        &= \alpha\langle \nabla\phi_t(z_t), g_t \rangle - \frac{L\alpha^2}{2}\|g_t\|^2 \\
        &= \alpha\|\nabla\phi_t(z_t)\|^2 + \alpha\langle \nabla\phi_t(z_t), \varepsilon_t \rangle - \frac{L\alpha^2}{2}(\|\nabla\phi_t(z_t)\|^2 + 2\langle \nabla\phi_t(z_t), \varepsilon_t \rangle + \|\varepsilon_t\|^2) \\
        &= \frac{\alpha}{2}(2-L\alpha)\|\nabla\phi_t(z_t)\|^2 - \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle,
    \end{aligned}
\end{equation}
where we use $g_t = \nabla\phi_t(z_t) + \varepsilon_t$ in the second equality. Noting that by \eqref{eq:NAG-single} we have
\begin{equation*}
    w_t-z_t = -\gamma(w_t-w_t^*) + \gamma(w_{t-1}-w_t^*),
\end{equation*}
and combining \eqref{eq:phi-t-SC} and \eqref{eq:phi-t-smooth} we obtain 
\begin{equation} \label{eq:X_1}
    \begin{aligned}
        \phi_t(w_t) - \phi_t(w_{t+1}) 
        &\geq \langle \nabla\phi_t(z_t), w_t-z_t \rangle + \frac{\mu}{2}\|w_t-z_t\|^2 \\
        &\quad+ \frac{\alpha}{2}(2-L\alpha)\|\nabla\phi_t(z_t)\|^2 - \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle \\
        &= 
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}^{\top}
        \rmX_1
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}
        - \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle,
    \end{aligned}
\end{equation}
where matrix $\rmX_1\in\R^{3d\times3d}$ is defined as
% where matrix $\rmX_1\in\R^{4d\times4d}$ is defined as
% \begin{equation*}
%     \rmX_1 = \frac{1}{2}
%     \begin{bmatrix}
%         \mu\gamma^2 & -\mu\gamma^2 & -\gamma & 0 \\
%         -\mu\gamma^2 & \mu\gamma^2 & \gamma & 0 \\
%         -\gamma & \gamma & \alpha(2-L\alpha) & 0 \\
%         0 & 0 & 0 & 0
%     \end{bmatrix} \otimes \rmI_d.
% \end{equation*}
\begin{equation*}
    \rmX_1 = \frac{1}{2}
    \begin{bmatrix}
        \mu\gamma^2 & -\mu\gamma^2 & -\gamma \\
        -\mu\gamma^2 & \mu\gamma^2 & \gamma \\
        -\gamma & \gamma & \alpha(2-L\alpha) \\
    \end{bmatrix} \otimes \rmI_d.
\end{equation*}
Then applying the strong convexity of $\phi_t$ again gives
\begin{equation} \label{eq:phi-t-SC-1}
    \phi_t(w_t^*) - \phi_t(z_t) \geq \langle \nabla\phi_t(z_t), w_t^*-z_t \rangle + \frac{\mu}{2}\|w_t^*-z_t\|^2.
\end{equation}
Noting that
\begin{equation*}
    \begin{aligned}
        w_t^* - z_t
        &= (w_t^*-w_t) - \gamma(w_t-w_t^*) + \gamma(w_{t-1}-w_t^*) \\
        &= -(1+\gamma)(w_t-w_t^*) + \gamma(w_{t-1}-w_t^*),
    \end{aligned}
\end{equation*}
and combining \eqref{eq:phi-t-smooth} and \eqref{eq:phi-t-SC-1} we obtain
\begin{equation} \label{eq:X_2}
    \begin{aligned}
        \phi_t(w_t^*) - \phi_t(w_{t+1}) 
        &\geq \langle \nabla\phi_t(z_t), w_t^*-z_t \rangle + \frac{\mu}{2}\|w_t^*-z_t\|^2 \\
        &\quad+ \frac{\alpha}{2}(2-L\alpha)\|\nabla\phi_t(z_t)\|^2 - \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle \\
        &= 
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}^{\top}
        \rmX_2
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}
        - \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle,
    \end{aligned}
\end{equation}
where matrix $\rmX_2\in\R^{3d\times3d}$ is defined as
% where matrix $\rmX_2\in\R^{4d\times4d}$ is defined as
% \begin{equation*}
%     \rmX_2 = \frac{1}{2}
%     \begin{bmatrix}
%         \mu(1+\gamma)^2 & -\mu\gamma(1+\gamma) & -(1+\gamma) & 0 \\
%         -\mu\gamma(1+\gamma) & \mu\gamma^2 & \gamma & 0 \\
%         -(1+\gamma) & \gamma & \alpha(2-L\alpha) & 0 \\
%         0 & 0 & 0 & 0
%     \end{bmatrix} \otimes \rmI_d.
% \end{equation*}
\begin{equation*}
    \rmX_2 = \frac{1}{2}
    \begin{bmatrix}
        \mu(1+\gamma)^2 & -\mu\gamma(1+\gamma) & -(1+\gamma) \\
        -\mu\gamma(1+\gamma) & \mu\gamma^2 & \gamma \\
        -(1+\gamma) & \gamma & \alpha(2-L\alpha) \\
    \end{bmatrix} \otimes \rmI_d.
\end{equation*}
Next, we multiply \eqref{eq:X_1} by $\rho^2$ and \eqref{eq:X_2} by $1-\rho^2$, then sum them up to get
\begin{equation} \label{eq:multiply-step}
    \begin{aligned}
        \rho^2(\phi_t(w_t)&-\phi_t(w_t^*)) - (\phi_t(w_{t+1})-\phi_t(w_t^*)) \\
        &\geq 
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}^{\top}
        (\rho^2\rmX_1 + (1-\rho^2)\rmX_2)
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}
        - \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle.
    \end{aligned}
\end{equation}
% With definition of $\gamma,\rho^2$ and $\rmP$ given in the statement of the theorem, by direct calculation we have
% \begin{equation*}
%     \begin{aligned}
%         &
%         \begin{bmatrix}
%             \rmA^{\top}\rmP\rmA-\rho^2\rmP & \rmA^{\top}\rmP\rmB \\
%             \rmB^{\top}\rmP\rmA & \rmB^{\top}\rmP\rmB
%         \end{bmatrix}
%         - (\rho^2\rmX_1 + (1-\rho^2)\rmX_2) \\
%         &\quad\quad\quad\quad\quad= 
%         \begin{bmatrix}
%             -\frac{\mu(1-\sqrt{\mu\alpha})^3}{2\sqrt{\mu\alpha}(1+\sqrt{\mu\alpha})} & \frac{\mu(1-\sqrt{\mu\alpha})^3}{2\sqrt{\mu\alpha}(1+\sqrt{\mu\alpha})} & 0 & -\frac{1+\mu\alpha}{2(1+\sqrt{\mu\alpha})} \\
%             \frac{\mu(1-\sqrt{\mu\alpha})^3}{2\sqrt{\mu\alpha}(1+\sqrt{\mu\alpha})} & -\frac{\mu(1-\sqrt{\mu\alpha})^3}{2\sqrt{\mu\alpha}(1+\sqrt{\mu\alpha})} & 0 & \frac{1-\sqrt{\mu\alpha}}{2(1+\sqrt{\mu\alpha})} \\
%             0 & 0 & -\frac{\alpha(1-L\alpha)}{2} & \frac{\alpha}{2} \\
%             -\frac{1+\mu\alpha}{2(1+\sqrt{\mu\alpha})} & \frac{1-\sqrt{\mu\alpha}}{2(1+\sqrt{\mu\alpha})} & \frac{\alpha}{2} & \frac{\alpha}{2}
%         \end{bmatrix} \otimes \rmI_d
%         := \rmC,
%     \end{aligned}
% \end{equation*}
% where matrix $\rmC$ is negative semidefinite \cite{chen2023convergence}, i.e., $\rmC\preceq\mathbf{0}$. Then we use this fact to get
By \cite[Corollary 4.9]{aybat2020robust} (see also \cite[Theorem 2.3]{aybat2019universally}), we have the following fact:
\begin{equation} \label{eq:nsd-fact}
    \begin{aligned}
        \begin{bmatrix}
            \rmA^{\top}\rmP\rmA-\rho^2\rmP & \rmA^{\top}\rmP\rmB \\
            \rmB^{\top}\rmP\rmA & \rmB^{\top}\rmP\rmB
        \end{bmatrix}
        - (\rho^2\rmX_1 + (1-\rho^2)\rmX_2)
        \preceq 0,
    \end{aligned}
\end{equation}
which, combined with \eqref{eq:multiply-step} yields
\begin{equation*}
    \begin{aligned}
        &
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}
        - \rho^2\theta_t^{\top}\rmP\theta_t
        = 
        % \begin{bmatrix}
        %     \theta_t \\
        %     \omega_t
        % \end{bmatrix}^{\top}
        % (\rho^2\rmX_1 + (1-\rho^2)\rmX_2 + \rmC)
        % \begin{bmatrix}
        %     \theta_t \\
        %     \omega_t
        % \end{bmatrix} \\
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}^{\top}
        \begin{bmatrix}
            \rmA^{\top}\rmP\rmA-\rho^2\rmP & \rmA^{\top}\rmP\rmB \\
            \rmB^{\top}\rmP\rmA & \rmB^{\top}\rmP\rmB
        \end{bmatrix}
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix} \\
        &\quad\quad\leq 
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix}^{\top}
        (\rho^2\rmX_1 + (1-\rho^2)\rmX_2)
        \begin{bmatrix}
            \theta_t \\
            \omega_t
        \end{bmatrix} \\
        &\quad\quad\leq- (\phi_t(w_{t+1})-\phi_t(w_t^*)) + \rho^2(\phi_t(w_t)-\phi_t(w_t^*)) - \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2,
    \end{aligned}
\end{equation*}
where the first inequality uses \eqref{eq:nsd-fact}, and the last inequality follows by \eqref{eq:multiply-step}. Rearrange the above inequality and by definition of the potential function $V_t$, we obtain
\begin{equation} \label{eq:nag-one-step}
    \begin{aligned}
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}
        &+ \phi_t(w_{t+1}) - \phi_t(w_t^*) \\
        &\leq \rho^2V_t - \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2.
    \end{aligned}
\end{equation}
Now recall that in \eqref{eq:obj-time-drift} our objective function has the form of $\phi_t(w) = \frac{\mu}{2}\|w-w_t^*\|^2$, hence $\nabla\phi_t(z_t) = \mu(z_t-w_t^*)$. Plugging this into the above inequality gives
\begin{equation}
    \begin{aligned}
        &\begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}^{\top}
        \rmP
        \begin{bmatrix}
            w_{t+1} - w_t^* \\
            w_t - w_t^* 
        \end{bmatrix}
        + \phi_t(w_{t+1}) - \phi_t(w_t^*) \\
        &\quad\quad\leq \rho^2V_t - \mu\alpha(1-L\alpha)\langle z_t-w_t^*, \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 \\
        &\quad\quad= \rho^2V_t - \mu\alpha(1-L\alpha)\langle w_t-w_t^*, \varepsilon_t \rangle - \mu\alpha(1-L\alpha)\langle z_t-w_t, \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 \\
        &\quad\quad= \rho^2V_t - \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \\
        &\quad\quad\quad\quad\quad\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2,
    \end{aligned}
\end{equation}
where $u_{t,1}$ and $u_{t,2}$ are defined as
\begin{equation*}
    u_{t,1} = \frac{w_t-w_t^*}{\|w_t-w_t^*\|},
    \quad\quad
    u_{t,2} = \frac{z_t-w_t}{\|z_t-w_t\|}.
\end{equation*}
Therefore, we conclude that
\begin{equation} \label{eq:bound-A}
    \begin{aligned}
        (A) 
        &\leq \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)
        \left[\rho^2V_t - \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad\quad\quad\quad\quad\quad\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] \\
        &\leq \left(1-\frac{3\sqrt{\mu\alpha}}{4}\right)V_t + 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad\quad\quad\quad\quad\quad\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right], \\
    \end{aligned}
\end{equation}
where the last inequality follows from the definition of $\rho$ and simple calculation
\begin{equation*}
    \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\rho^2
    = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)(1-\sqrt{\mu\alpha})
    \leq 1-\frac{3\sqrt{\mu\alpha}}{4}.
\end{equation*}

\paragraph{Bounding $(B)$.}
Recall that under distributional drift, the objective function in \eqref{eq:obj-time-drift} has the form of $\phi_t(w) = \frac{\mu}{2}\|w-w_t^*\|^2$, then we have
\begin{equation*}
    \begin{aligned}
        (B) 
        &= \phi_{t+1}(w_{t+1}) - \phi_{t+1}(w_{t+1}^*) - \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)(\phi_t(w_{t+1}) - \phi_t(w_t^*)) \\
        &\leq \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)(\phi_{t+1}(w_{t+1}) - \phi_{t+1}(w_{t+1}^*) - \phi_t(w_{t+1}) + \phi_t(w_t^*)) \\
        &= \frac{\mu}{2}\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)(\|w_{t+1}-w_{t+1}^*\|^2 - \|w_{t+1}-w_t^*\|^2) \\
        &\leq \frac{\mu}{2}\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\|w_t^*-w_{t+1}^*\|\|w_{t+1}-w_t^*+w_{t+1}-w_{t+1}^*\| \\
        &\leq \frac{\mu}{2}\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\Delta_t(2\|w_{t+1}-w_{t+1}^*\| + \|w_{t+1}^*-w_t^*\|) \\
    \end{aligned}
\end{equation*}
Since $\phi_{t+1}$ is $\mu$-strongly convex and matrix $\rmP$ is PSD, then 
\begin{equation*}
    \begin{aligned}
        V_{t+1} 
        &= \theta_{t+1}^{\top}\rmP\theta_{t+1} + \phi_{t+1}(w_{t+1}) - \phi_t(w_{t+1}^*)
        \geq \phi_{t+1}(w_{t+1}) - \phi_t(w_{t+1}^*) \\
        &\geq \frac{\mu}{2}\|w_{t+1}-w_{t+1}^*\|^2
        \quad\quad\quad\quad\Longrightarrow\quad\quad\quad\quad
        \|w_{t+1}-w_{t+1}^*\| \leq \sqrt{\frac{2}{\mu}}\sqrt{V_{t+1}}.
    \end{aligned}
\end{equation*}
Plugging the above fact back into the upper bound for $(B)$ gives
\begin{equation} \label{eq:bound-B}
    \begin{aligned}
        (B)
        &\leq \frac{\mu}{2}\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\Delta_t\left(2\sqrt{\frac{2}{\mu}}\sqrt{V_{t+1}} + \Delta_t\right) \\
        &= \sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\sqrt{V_{t+1}} + \frac{\mu}{2}\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\Delta_t^2.
    \end{aligned}
\end{equation}

\paragraph{Bounding $(C)$.}
For this part, we handle the distributional drift. By definition of $\rmP$ in \eqref{eq:gamma-rhp-P}, we have
% Recall that under this condition we consider one-dimensional case, that is, we let $d=1$ in \eqref{eq:obj-time-drift} such that $w\in\R$. Then we use $\rmP\in\R^{2\times2}$ to obtain
\begin{equation} \label{eq:bound-C}
    \begin{aligned}
        (C)
        &= \left(1+\frac{4}{\sqrt{\mu\alpha}}\right)
        \begin{bmatrix}
            w_t^* - w_{t+1}^* \\
            w_t^* - w_{t+1}^*
        \end{bmatrix}^{\top}
        \frac{1}{2\alpha}
        \begin{bmatrix}
        \rmI_{d} & (\sqrt{\mu\alpha}-1)\rmI_{d} \\
        (\sqrt{\mu\alpha}-1)\rmI_{d} & (1-\sqrt{\mu\alpha})^2\rmI_{d}
        \end{bmatrix}
        \begin{bmatrix}
            w_t^* - w_{t+1}^* \\
            w_t^* - w_{t+1}^*
        \end{bmatrix} \\
        &= \frac{\mu}{2}\left(1+\frac{4}{\sqrt{\mu\alpha}}\right)\Delta_t^2, 
    \end{aligned}
\end{equation}
where in the last equality we use the basic algebra of block matrix multiplication and the definition of $\Delta_t= \|w_t^*-w_{t+1}^*\|$.
% the fact that 
% \begin{equation}
% \| w_t^* - w_{t+1}^*\|^2=\Delta_t^2.
% \end{equation}

\paragraph{Final Bound for $V_{t+1}$.}
Now we are ready to derive the upper bound for $V_{t+1}$. Combining \eqref{eq:bound-A}, \eqref{eq:bound-B} and \eqref{eq:bound-C} together yields
\begin{equation} \label{eq:bound-V(t+1)-1}
    \begin{aligned}
        V_{t+1}
        &\leq (A) + (B) + (C) \\
        &\leq \left(1-\frac{3\sqrt{\mu\alpha}}{4}\right)V_t + 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad\quad\quad\quad\quad\quad\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] \\
        &\quad+ \sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\sqrt{V_{t+1}} + \mu\left(1+\frac{\sqrt{\mu\alpha}}{8}+\frac{2}{\sqrt{\mu\alpha}}\right)\Delta_t^2.
    \end{aligned}
\end{equation}
For simplicity, we define $D$ as the following 
\begin{equation*}
    \begin{aligned}
        D 
        &= \left(1-\frac{3\sqrt{\mu\alpha}}{4}\right)V_t + 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] + \mu\left(1+\frac{\sqrt{\mu\alpha}}{8}+\frac{2}{\sqrt{\mu\alpha}}\right)\Delta_t^2.
    \end{aligned}
\end{equation*}
Hence \eqref{eq:bound-V(t+1)-1} turns into
\begin{equation*}
    \begin{aligned}
        V_{t+1} - \sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\sqrt{V_{t+1}} - D \leq 0.
    \end{aligned}
\end{equation*}
Solving the above inequality we get
\begin{equation*}
    \begin{aligned}
        \sqrt{V_{t+1}}
        &\leq \frac{1}{2}\left[\sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right) + \sqrt{\left(\sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\right)^2 + 4D}\right] \\
        &\leq \sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right) + \sqrt{D} 
    \end{aligned}
\end{equation*}
Then an application of Young's inequality reveals
\begin{equation*}
    \begin{aligned}
        V_{t+1}
        &\leq \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)D + \left(1+\frac{4}{\sqrt{\mu\alpha}}\right)\left(\sqrt{2\mu}\Delta_t\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\right)^2 \\
        &= \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\left\{
        \left(1-\frac{3\sqrt{\mu\alpha}}{4}\right)V_t + 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\right.\\
        &\left.\left.\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] + \mu\left(1+\frac{\sqrt{\mu\alpha}}{8}+\frac{2}{\sqrt{\mu\alpha}}\right)\Delta_t^2
        \right\} \\
        &\quad+ \left(1+\frac{4}{\sqrt{\mu\alpha}}\right)2\mu\Delta_t^2\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)^2 \\
        &\leq \left(1-\frac{\sqrt{\mu\alpha}}{2}\right)V_t + \left(1+\frac{\sqrt{\mu\alpha}}{4}\right) 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] \\
        &\quad+ \mu\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\left(1+\frac{\sqrt{\mu\alpha}}{8}+\frac{2}{\sqrt{\mu\alpha}}\right)\Delta_t^2 + \left(1+\frac{4}{\sqrt{\mu\alpha}}\right)2\mu\Delta_t^2\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)^2,
    \end{aligned}
\end{equation*}
where we plug in the definition of $D$ for the first equality. 
Since the learning rate $\alpha\leq 1/L$ and thus $\mu\alpha\leq 1$, then we have
\begin{equation*}
    \begin{aligned}
        \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\left(1+\frac{\sqrt{\mu\alpha}}{8}+\frac{2}{\sqrt{\mu\alpha}}\right) \leq \frac{125}{32\sqrt{\mu\alpha}},
        \quad\quad
        2\left(1+\frac{4}{\sqrt{\mu\alpha}}\right)\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)^2 
        \leq \frac{125}{8\sqrt{\mu\alpha}}.
    \end{aligned}
\end{equation*}
Therefore, we finally conclude that
\begin{equation*}
    \begin{aligned}
        V_{t+1}
        &\leq \left(1-\frac{\sqrt{\mu\alpha}}{2}\right)V_t + \left(1+\frac{\sqrt{\mu\alpha}}{4}\right) 
        \left[- \sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad\quad- \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] + \frac{20\mu\Delta_t^2}{\sqrt{\mu\alpha}},
    \end{aligned}
\end{equation*}
which is as claimed in \eqref{eq:one-step-single-level}.
\end{proof}


When there is no drift, the following lemma holds for any general strongly convex functions $\phi$ in  $\R^d$.

\begin{lemma}[Distance recursion, without drift] \label{lm:dist-without-drift}
Under the same settings as in \Cref{lm:distance-recursion-single-level} with $\phi_t(w)\equiv \phi(w)$, 
% $w\in\R^d$, 
and $w_t^*\equiv w^*$, where $\phi(w)$ can be any general strongly functions in $\R^d$. We redefine $u_{t,1}, u_{t,2}$ as 
\begin{equation} 
    u_{t,1} = \frac{\nabla\phi(w_t)-\nabla\phi(w^*)}{\|\nabla\phi(w_t)-\nabla\phi(w^*)\|},
    \quad\quad
    u_{t,2} = \frac{\nabla\phi(z_t)-\nabla\phi(w_t)}{\|\nabla\phi(z_t)-\nabla\phi(w_t)\|}.
\end{equation}
Then for all $t\geq0$, it holds that
\begin{equation} 
    \begin{aligned}
        V_{t+1}
        &\leq (1-\sqrt{\mu\alpha})V_t - \sqrt{\frac{2}{\mu}}L\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\frac{1}{L}\sqrt{\frac{\mu}{2}}\|\nabla\phi_t(w_t)-\nabla\phi_t(w^*)\| \\
        &\quad\quad- \frac{2L\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2L\sqrt{2\alpha}}\|\nabla\phi_t(z_t)-\nabla\phi_t(w_t)\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2.
    \end{aligned}
\end{equation}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:dist-without-drift}]
By \eqref{eq:all-d} in \Cref{lm:distance-recursion-single-level} with $\phi_t(w)\equiv \phi(w)$ and $w_t^*\equiv w^*$, we have
\begin{equation*}
    \begin{aligned}
        V_{t+1} 
        &\leq \rho^2V_t - \alpha(1-L\alpha)\langle \nabla\phi_t(z_t), \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 \\
        &= \rho^2V_t - \alpha(1-L\alpha)\langle \nabla\phi_t(w_t)-\nabla\phi_t(w^*), \varepsilon_t \rangle - \alpha(1-L\alpha)\langle \nabla\phi_t(z_t)-\nabla\phi_t(w_t), \varepsilon_t \rangle + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2 \\
        &= (1-\sqrt{\mu\alpha})V_t - \sqrt{\frac{2}{\mu}}L\alpha(1-L\alpha)\langle u_{t,1}, \varepsilon_t \rangle\frac{1}{L}\sqrt{\frac{\mu}{2}}\|\nabla\phi_t(w_t)-\nabla\phi_t(w^*)\| \\
        &\quad\quad- \frac{2L\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, \varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2L\sqrt{2\alpha}}\|\nabla\phi_t(z_t)-\nabla\phi_t(w_t)\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2.
    \end{aligned}
\end{equation*}
Hence the proof is completed.
\end{proof}


The following result shows the first part of \Cref{lm:option-1-single}. To the best of our knowledge, this is the first high probability guarantee with improved rate for SNAG under distributional drift.

\begin{lemma}[High-probability distance tracking, with drift] \label{lm:dist-track-single-level} 
Under the same setting as in \Cref{lm:distance-recursion-single-level} with $\alpha\leq \min\{1/2L, \mu/2L^2, 1/10^3\mu\}$, for any given $\delta\in(0,1)$ and all $t\in[T]$, the following holds with probability at least $1-\delta$ over the randomness in $\gH_t$:
\begin{equation}
    V_t \leq \left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^tV_0 + \left(2\alpha\sigma^2 + \frac{80\Delta^2}{\alpha}\right)\ln\frac{eT}{\delta}.
\end{equation}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:dist-track-single-level}]
We will invoke \Cref{lm:recursive-control} to show the results. 
To apply \Cref{lm:recursive-control}, we first need to show the following two facts:
\begin{equation} \label{eq:less-Vt}
    \begin{aligned}
        \text{Fact (I)}:\quad \sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \leq \sqrt{V_t}
        \quad\quad\&\quad\quad
        \text{Fact (II)}:\quad \frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| \leq \sqrt{V_t}.
    \end{aligned}
\end{equation}

\paragraph{Fact (I) verification.}
Since $\phi_t$ is $\mu$-strongly convex and matrix $\rmP$ is PSD, then 
\begin{equation*}
    \begin{aligned}
        V_t
        &= \theta_t^{\top}\rmP\theta_t + \phi_t(w_t) - \phi_t(w_t^*)
        \geq \phi_t(w_t) - \phi_t(w_t^*) \\
        &\geq \frac{\mu}{2}\|w_t-w_t^*\|^2
        \quad\quad\quad\quad\Longrightarrow\quad\quad\quad\quad
        \sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \leq \sqrt{V_t}.
    \end{aligned}
\end{equation*}

\paragraph{Fact (II) verification.}
By definition of matrix $\rmP$ and simple calculation we have
\begin{equation*}
    \begin{aligned}
        \sqrt{V_t}
        &\geq \sqrt{\theta_t^{\top}\rmP\theta_t} 
        = \sqrt{\frac{1}{2\alpha}}\|(w_t-w_t^*) + (\sqrt{\mu\alpha}-1)(w_{t-1}-w_t^*)\| \\
        &= \sqrt{\frac{1}{2\alpha}}\|(1-\sqrt{\mu\alpha})(w_t-w_{t-1}) + \sqrt{\mu\alpha}(w_t-w_t^*)\| \\
        &\geq \sqrt{\frac{1}{2\alpha}}(1-\sqrt{\mu\alpha})\|w_t-w_{t-1}\| - \sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \\
        &\geq \sqrt{\frac{1}{2\alpha}}(1-\sqrt{\mu\alpha})\|w_t-w_{t-1}\| - \sqrt{V_t}.
    \end{aligned}
\end{equation*}
Rearrange the above inequality, and recall the update rule of stochastic Nesterov accelerated gradient method, we have
\begin{equation*}
    \begin{aligned}
        \|z_t-w_t\|
        &= \gamma\|w_t-w_{t-1}\|
        \leq \frac{2\gamma\sqrt{2\alpha}}{1-\sqrt{\mu\alpha}}\sqrt{V_t} 
        = \frac{2\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\sqrt{V_t},
    \end{aligned}
\end{equation*}
where for the last equality we use the definition of $\gamma$ as in \eqref{eq:gamma-rhp-P}. Rearrange it gives \eqref{eq:less-Vt}.

By \Cref{lm:distance-recursion-single-level} we have
\begin{equation} \label{eq:apply-control}
    \begin{aligned}
        V_{t+1}
        &\leq \left(1-\frac{\sqrt{\mu\alpha}}{2}\right)V_t + \left(1+\frac{\sqrt{\mu\alpha}}{4}\right) 
        \left[\sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, -\varepsilon_t \rangle\sqrt{\frac{\mu}{2}}\|w_t-w_t^*\| \right.\\
        &\left.\quad\quad+ \frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, -\varepsilon_t \rangle\frac{1+\sqrt{\mu\alpha}}{2\sqrt{2\alpha}}\|z_t-w_t\| + \frac{L\alpha^2}{2}\|\varepsilon_t\|^2\right] + \frac{20\mu\Delta_t^2}{\sqrt{\mu\alpha}}.
    \end{aligned}
\end{equation}
Note that under \Cref{ass:noise-drift-single-level}, there exists an absolute constant $c\geq1$ such that for all $t\geq0$, $\|\varepsilon_t\|^2$ is sub-exponential conditioned on $\gH_t$ with parameter $c\sigma^2$, and $\varepsilon_t$ is mean-zero sub-Gaussian conditioned on $\gH_t$ with parameter $c\sigma$ \cite[Theorem 30]{cutler2023stochastic}. For convenience we simply let $c=1$ here. Thus $\langle u_{t,1}, -\varepsilon_t \rangle$ is mean-zero sub-Gaussian conditioned on $\gH_t$ with parameter $\sigma$, and $\Delta_t^2$ is sub-exponential conditioned on $\gH_t$ with parameter $\Delta^2$ by assumption. Hence, in light of \eqref{eq:apply-control}, we apply \Cref{lm:recursive-control} with
\begin{equation*}
    \gH_t = \gH_t,
    \quad
    V_t = V_t,
    \quad
    V'_{t,1} = \frac{\mu}{2}\|w_t-w_t^*\|^2,
    \quad
    V'_{t,2} = \frac{(1+\sqrt{\mu\alpha})^2}{8\alpha}\|z_t-w_t\|^2,
\end{equation*}
\begin{equation*}
    D_{t,1} = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\sqrt{2\mu}\alpha(1-L\alpha)\langle u_{t,1}, -\varepsilon_t \rangle,
    \quad
    D_{t,2} = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\langle u_{t,2}, -\varepsilon_t \rangle,
\end{equation*}
\begin{equation*}
    X_t = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{L\alpha^2}{2}\|\varepsilon_t\|^2 + \frac{20\mu\Delta_t^2}{\sqrt{\mu\alpha}}, 
    \quad
    \alpha_t = 1-\frac{\sqrt{\mu\alpha}}{2},
    \quad
    \kappa_t = 0,
\end{equation*}
\begin{equation*}
    \sigma_1 = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\sqrt{2\mu}\alpha(1-L\alpha)\sigma,
    \quad
    \sigma_2 = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{2\mu\sqrt{2\alpha}}{1+\sqrt{\mu\alpha}}\alpha(1-L\alpha)\sigma,
\end{equation*}
\begin{equation*}
    \nu_t = \left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{L\alpha^2}{2}\sigma^2 + \frac{20\mu\Delta^2}{\sqrt{\mu\alpha}},
\end{equation*}
yielding the following recursion 
\begin{equation} \label{eq:recursion-dist}
    \begin{aligned}
        \E[\exp(\lambda V_{t+1})]
        &\leq \exp\left(\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{L\alpha^2}{2}\sigma^2 + \frac{20\mu\Delta^2}{\sqrt{\mu\alpha}}\right) \E\left[\exp\left(\lambda\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)V_t\right)\right]
    \end{aligned}
\end{equation}
for all $\lambda$ satisfying
\begin{equation*}
    0 \leq \lambda \leq
    \min\left\{\frac{2}{125\alpha\sqrt{\mu\alpha}\sigma^2}, \frac{1}{5\alpha\sigma^2/4 + 40\mu\Delta^2/\sqrt{\mu\alpha}}\right\}.
\end{equation*}
We then apply \eqref{eq:recursion-dist} recursively to deduce
\begin{equation*}
    \begin{aligned}
        \E[\exp(\lambda V_{t+1})]
        &\leq \exp\left[\lambda\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^tV_0 + \lambda\left(\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{L\alpha^2}{2}\sigma^2 + \frac{20\mu\Delta^2}{\sqrt{\mu\alpha}}\right)\sum_{i=0}^{t-1}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^{i}\right] \\
        &\leq \exp\left\{\lambda\left[\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^tV_0 + 2\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{L\alpha^2}{\sqrt{\mu\alpha}}\sigma^2 + \frac{80\Delta^2}{\alpha}\right]\right\}
    \end{aligned}
\end{equation*}
for all $\lambda$ satisfying
\begin{equation*}
    0 \leq \lambda \leq
    \min\left\{\frac{2}{125\alpha\sqrt{\mu\alpha}\sigma^2}, \frac{1}{5\alpha\sigma^2/4 + 40\mu\Delta^2/\sqrt{\mu\alpha}}\right\}.
\end{equation*}
Moreover, setting
\begin{equation*}
    \nu \coloneqq 2\alpha\sigma^2 + \frac{80\Delta^2}{\alpha}
\end{equation*}
and taking into account $\alpha\leq \min\{1/2L, \mu/2L^2, 1/10^3\mu\}$, then we have
\begin{equation*}
    2\left(1+\frac{\sqrt{\mu\alpha}}{4}\right)\frac{L\alpha^2}{\sqrt{\mu\alpha}}\sigma^2 + \frac{80\Delta^2}{\alpha} \leq \nu
\end{equation*}
and
\begin{equation*}
    \frac{1}{\nu} = \frac{1}{2\alpha\sigma^2 + 80\Delta^2/\alpha} 
    \leq \min\left\{\frac{2}{125\alpha\sqrt{\mu\alpha}\sigma^2}, \frac{1}{5\alpha\sigma^2/4 + 40\mu\Delta^2/\sqrt{\mu\alpha}}\right\}.
\end{equation*}
Thus we obtain
\begin{equation*}
    \begin{aligned}
        \E\left[\exp\left(\lambda\left(V_t - \left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^tV_0\right)\right)\right] \leq \exp(\lambda\nu)
        \quad\text{for all}\quad 0\leq \lambda\leq 1/\nu.
    \end{aligned}
\end{equation*}
Taking $\lambda=1/\nu$ and applying Markov's inequality and union bound completes the proof.
\end{proof}


The following result shows the second part of \Cref{lm:option-1-single}.

\begin{lemma}[High-probability distance tracking, without drift] \label{lm:track-without-drift}
Under the same setting as in \Cref{lm:dist-without-drift} with $\alpha\leq \min\{1/2L, \mu/10^3L^2\}$, for any given $\delta\in(0,1)$ and all $t\in[T]$, the following holds with probability at least $1-\delta$ over the randomness in $\gH_t$:
\begin{equation}
    V_t \leq \left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^tV_0 + 2\alpha\sigma^2 \ln\frac{eT}{\delta}.
\end{equation}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:track-without-drift}]
First it is easy to verify that 
\begin{equation*}
    \frac{1}{L}\sqrt{\frac{\mu}{2}}\|\nabla\phi_t(w_t)-\nabla\phi_t(w^*)\| \leq \sqrt{V_t}
    \quad\quad\text{and}\quad\quad
    \frac{1+\sqrt{\mu\alpha}}{2L\sqrt{2\alpha}}\|\nabla\phi_t(z_t)-\nabla\phi_t(w_t)\| \leq \sqrt{V_t}.
\end{equation*}
Then we apply \Cref{lm:recursive-control} to obtain the final result. We omit the detailed proof here since it follows the same procedure as in proof of \Cref{lm:dist-track-single-level}.
\end{proof}

==> proof_sketch_2.tex <==
We first present the following algebraic fact under suitable choice of parameters.

\begin{lemma}[Parameter choice, informal] \label{lm:parameter-choice}
For any given $\delta\in(0,1)$ and any small $\epsilon$ satisfying 
\begin{equation} \label{eq:para-eps}
    \begin{aligned}
        \epsilon \leq \left(\frac{164\cdot32ed_0L_0^2\sigma_{g,1}^2}{\delta\mu^2}\max\left\{\frac{l_{g,1}}{\sigma_{g,1}}, \frac{\Bar{\sigma}}{d_0}\right\}\right)^{1/3},
    \end{aligned}
\end{equation}
if we set parameters $\alpha,\beta,\eta, T$ as 
\begin{equation} \label{eq:para}
    1-\beta = \frac{\mu^2\epsilon^2}{164\cdot16L_0^2\sigma_{g,1}^2\ln(P)},
    \quad
    \eta = \min\left\{\frac{\sigma_{g,1}}{l_{g,1}}, \frac{d_0}{\Bar{\sigma}}\right\}(1-\beta), 
    \quad
    \alpha = \frac{1}{\mu}(1-\beta),
    \quad
    T = \frac{4d_0}{\eta\epsilon},
\end{equation}
where $\Bar{\sigma}$ is defined in \Cref{lm:hyper-var}, and $d_0$ and $P$ are defined as
\begin{equation} \label{eq:d0-P}
    d_0=\Phi(x_0)-\inf_{x\in\R^{d_x}}\Phi(x),
    \quad
    P = \left(\frac{164\cdot64ed_0L_0^2\sigma_{g,1}^2}{\delta\mu^2\epsilon^3}\max\left\{\frac{l_{g,1}}{\sigma_{g,1}}, \frac{\Bar{\sigma}}{d_0}\right\}\right)^2.
\end{equation}
Then the following holds for all $t\in[T]$:
\begin{equation*}
    \left(\frac{4\alpha\sigma_{g,1}^2}{\mu} + \frac{160\eta^2l_{g,1}^2}{\mu^3\alpha}\right)\ln\frac{eT}{\delta} \leq \frac{\epsilon^2}{16L_0^2}.
\end{equation*}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:parameter-choice}]
By \Cref{lm:lip-y*z*}, we have $\Delta_t = \|y_t^*-y_{t+1}^*\| \leq \frac{l_{g,1}}{\mu}\|x_t-x_{t+1}\| = \eta l_{g,1}/\mu$. Thus in our bilevel setting, we choose $\Delta = \eta l_{g,1}/\mu$, where $\Delta$ is defined in \Cref{sec:nesterov}.
By choice of $\alpha,\eta,T$ as in \eqref{eq:para}, we have
\begin{equation*}
    \begin{aligned}
        \left(\frac{4\alpha\sigma_{g,1}^2}{\mu} + \frac{160\eta^2l_{g,1}^2}{\mu^3\alpha}\right)\ln\frac{eT}{\delta} 
        &= \left(\frac{4(1-\beta)\sigma_{g,1}^2}{\mu^2} + \frac{160\eta^2l_{g,1}^2}{\mu^2(1-\beta)}\right)\ln\left(\frac{4ed_0}{\delta\eta\epsilon}\right) \\
        &\leq \frac{164(1-\beta)\sigma_{g,1}^2}{\mu^2}\ln\left(\frac{4ed_0}{\delta\epsilon(1-\beta)}\max\left\{\frac{l_{g,1}}{\sigma_{g,1}}, \frac{\Bar{\sigma}}{4d_0}\right\}\right).
    \end{aligned}
\end{equation*}
Now we choose $\beta$ to be 
\begin{equation*}
    \begin{aligned}
        1-\beta = \frac{\mu^2\epsilon^2}{164\cdot16L_0^2\sigma_{g,1}^2\ln(P)}, 
        \quad\text{where}\quad
        P = \left(\frac{164\cdot64ed_0L_0^2\sigma_{g,1}^2}{\delta\mu^2\epsilon^3}\max\left\{\frac{l_{g,1}}{\sigma_{g,1}}, \frac{\Bar{\sigma}}{d_0}\right\}\right)^2.
    \end{aligned}
\end{equation*}
Then we have
\begin{equation*}
    \begin{aligned}
        \frac{164(1-\beta)\sigma_{g,1}^2}{\mu^2}\ln\left(\frac{4ed_0l_{g,1}}{\delta\epsilon\sigma_{g,1}(1-\beta)}\right)
        = \frac{\epsilon^2}{16L_0^2\ln(P)}\ln\left(\sqrt{P}\ln(P)\right)
        \leq \frac{\epsilon^2}{16L_0^2},
    \end{aligned}
\end{equation*}
where we use the fact that $\ln(\sqrt{P}\ln(P)) \leq \ln(P) \leq \ln^2(P)$ for any $P\geq 4$ by choice of $\epsilon$ as in \eqref{eq:para-eps}.
\end{proof}


In the rest of this section, we assume \Cref{ass:relax-smooth},~\ref{ass:f-and-g},~\ref{ass:noise} and~\ref{ass:individual-noise} hold. In addition, the failure probability $\delta\in(0,1)$ and $\epsilon>0$ are chosen in the same way as in \Cref{thm:main}. 

\subsection{Proof of \Cref{lem:warmstart}}

\begin{lemma}[Warm-start, Restatement of \Cref{lem:warmstart}] \label{eq:warm-start}
Let $\{y_t^{\init}\}$ be the iterates produced by line 2 of \Cref{alg:bilevel}. Set $\alpha^{\init}=\mu\alpha/(\mu+l_{g,1})=\widetilde{\Theta}(\epsilon^2)$ with $\alpha$ defined in \eqref{eq:para} and $\phi_t(y)\equiv g(x_0,y)$. Then $\|y_{T_0}^{\init}-y_0^*\| \leq \sqrt{\frac{\mu}{8(\mu+l_{g,1})}}\frac{\epsilon}{L_0}$ holds with probability at least $1-\delta$ over the randomness in $\widetilde{\mathcal{F}}^{\init}$ (we denote this event as $\gE_{\init}$) in $T_0=\widetilde{O}(1/\epsilon)$ iterations, where
\begin{equation}
    T_0 = \ln\left(\frac{\mu^2\epsilon^2}{8(\mu+l_{g,1})^2L_0^2\|y_0^{\init}-y_0^*\|^2}\right) 
    \Big/
    \ln\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)
    = \widetilde{O}(1/\epsilon).
\end{equation}
\end{lemma}

\begin{proof}[Proof of \Cref{eq:warm-start}]
By \Cref{lm:track-without-drift}, \Cref{lm:parameter-choice} and $\mu$-strong convexity of $g$ in $y$, we have with probability at least $1-\delta$ over the randomness in $\gF^{\init}$ that
\begin{equation*}
    \begin{aligned}
        \|y_{T_0}^{\init}-y_0^*\|^2 
        &\leq \frac{2}{\mu}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^{T_0}U_0^{\init} + \frac{\mu}{\mu+l_{g,1}}\frac{4\alpha\sigma_{g,1}^2}{\mu}\ln\frac{eT_0}{\delta} \\
        &\leq \frac{2}{\mu}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^{T_0}U_0^{\init} + \frac{\mu}{\mu+l_{g,1}}\frac{\epsilon^2}{16L_0^2}.
    \end{aligned}
\end{equation*}
By $l_{g,1}$-smoothness of $g$ we have
\begin{equation*}
    \begin{aligned}
        U_0^{\init} 
        &= \frac{\mu}{2}\|y_0^{\init}-y_0^*\|^2 + g(x_0,y_0^{\init}) - g(x_0,y_0^*) \leq \frac{\mu+l_{g,1}}{2}\|y_0^{\init}-y_0^*\|^2.
    \end{aligned}
\end{equation*}
Now we set
\begin{equation*}
    \frac{2}{\mu}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^{T_0}\frac{\mu+l_{g,1}}{2}\|y_0^{\init}-y_0^*\|^2 + \frac{\mu}{\mu+l_{g,1}}\frac{\epsilon^2}{16L_0^2}
    \leq \frac{\mu}{\mu+l_{g,1}}\frac{\epsilon^2}{8L_0^2},
\end{equation*}
which gives
\begin{equation*}
    T_0 \geq \ln\left(\frac{\mu^2\epsilon^2}{8(\mu+l_{g,1})^2L_0^2\|y_0^{\init}-y_0^*\|^2}\right) 
    \Big/
    \ln\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)
\end{equation*}
By choice of $\alpha$ as in \eqref{eq:para} and simple calculation we obtain $T_0 = \widetilde{O}(1/\epsilon)$ when $\epsilon$ is small. 
\end{proof}


\subsection{Proof of \Cref{lem:optionI}}

\begin{lemma}[Option I, Restatement of \Cref{lem:optionI}] \label{lm:anytime-yt}
% Under \Cref{ass:relax-smooth},~\ref{ass:f-and-g},~\ref{ass:noise},~\ref{ass:individual-noise} and event $\gE_{\init}$, 
Under event $\gE_{\init}$, let $\{y_t\}$ be the iterates produced by Option I. Set $\alpha=\widetilde{\Theta}(\epsilon^2)$ as in \eqref{eq:para} and $\phi_t(y) = g(x_t,y) = \frac{\mu}{2}\|y-y_t^*\|^2$ with $y\in\R$. Then for any $t\in[T]$, \Cref{alg:bilevel} guarantees with probability at least $1-\delta$ over the randomness in $\widetilde{\mathcal{F}}_T^1$ (we denote this event as $\gE_y^1$) that $\|y_t-y_t^*\| \leq \epsilon/2L_0$.
\end{lemma}

\begin{proof}[Proof of \Cref{lm:anytime-yt}]
By \Cref{lm:dist-track-single-level} and~\ref{eq:warm-start} we have
\begin{equation*}
    \begin{aligned}
        \|y_t-y_t^*\|^2 
        &\leq \frac{2}{\mu}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^tU_0 + \left(\frac{4\alpha\sigma_{g,1}^2}{\mu} + \frac{160\eta^2l_{g,1}^2}{\mu^3\alpha}\right)\ln\frac{eT}{\delta} \\
        &= \frac{2}{\mu}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^t\left(\frac{\mu}{2}\|y_{T_0}^{\init}-y_0^*\|^2 + g(x_0,y_{T_0}^{\init}) - g(x_0,y_0^*)\right) + \left(\frac{4\alpha\sigma_{g,1}^2}{\mu} + \frac{160\eta^2l_{g,1}^2}{\mu^3\alpha}\right)\ln\frac{eT}{\delta} \\
        &\leq \frac{\mu+l_{g,1}}{\mu}\|y_{T_0}^{\init}-y_0^*\|^2 + \frac{\epsilon^2}{16L_0^2} 
        \leq \frac{3\epsilon^2}{16L_0^2}.
    \end{aligned}
\end{equation*}
Thus we conclude that for all $t\in[T]$, we have $\|y_t-y_t^*\| \leq \epsilon/2L_0$.
\end{proof}

\subsection{Proof of \Cref{lem:optionII}}

\begin{lemma}[Option II, Restatement of \Cref{lem:optionII}] \label{lm:periodic}
% Under \Cref{ass:relax-smooth},~\ref{ass:f-and-g},~\ref{ass:noise},~\ref{ass:individual-noise} and event $\gE_{\init}$, 
Under event $\gE_{\init}$, let $\{y_t\}$ be the iterates produced by Option II. set $\alpha'=\mu\alpha/(\mu+l_{g,1})=\widetilde{\Theta}(\epsilon^2)$ with $\alpha$ defined in \eqref{eq:para} and run SNAG in each update round for
\begin{equation}
    N = \ln\left(\frac{1}{8}\right) \Big/ \ln\left(1-\frac{\sqrt{\mu\alpha}}{4}\right) = \widetilde{O}(1/\epsilon)
\end{equation}
steps in every $I=\frac{\mu\epsilon}{2(1-\beta)L_0\sigma_{g,1}}=\widetilde{O}(1/\epsilon)$ iterations, set $\phi_t(y) = g(x_t,y)$ when $t$ is a multiple of $I$ (i.e., $x_t$ is fixed for each update round of Option II so $g$ can be general functions). Then for any $t\in[T]$, \Cref{alg:bilevel} guarantees with probability at least $1-\delta$ over the randomness in $\sigma(\cup_{t\leq T}\widetilde{\gF}_t^2)$ (we denote this event as $\gE_y^2$) that $\|y_t-y_t^*\| \leq \epsilon/L_0$. 
\end{lemma}

\begin{proof}[Proof of \Cref{lm:periodic}]
At the beginning of the first round, by \Cref{eq:warm-start} and~\ref{lm:anytime-yt} we have $\|y_0-y_0^*\|\leq \epsilon/2L_0$, then we do not update the lower-level variable until $t=I$-th iteration, then for $t=I$, we have
\begin{equation*}
    \begin{aligned}
        \|y_I-y_I^{*}\|
        &= \|y_0-y_I^*\|
        \leq \|y_0-y_0^*\| + \sum_{i=1}^{I}\|y_{i}^*-y_{i-1}^*\| \\
        &\leq \frac{\epsilon}{2L_0} + \frac{\eta l_{g,1}}{\mu}I
        = \frac{\epsilon}{L_0},
    \end{aligned}
\end{equation*}
where we plug in the definition of $\eta$ and $I$. 
By $l_{g,1}$-smoothness of $g$ we have
\begin{equation*}
    \begin{aligned}
        U_I
        &= \frac{\mu}{2}\|y_I-y_0^*\|^2 + g(x_I,y_I) - g(x_I,y_I^*) \leq \frac{\mu+l_{g,1}}{2}\|y_I-y_I^*\|^2 \leq \frac{\mu+l_{g,1}}{2}\frac{\epsilon^2}{L_0^2}
    \end{aligned}
\end{equation*}
Then for $N$ steps update in the inner loops of $t=I$-th iteration, we set
\begin{equation*}
    \frac{2}{\mu}\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)^{N}\frac{\mu+l_{g,1}}{2}\frac{\epsilon^2}{L_0^2} + \frac{\mu}{\mu+l_{g,1}}\frac{\epsilon^2}{16L_0^2}
    \leq \frac{\mu}{\mu+l_{g,1}}\frac{\epsilon^2}{8L_0^2},
\end{equation*}
which gives
\begin{equation*}
    N \geq \ln\left(\frac{1}{8}\right) \Big/ \ln\left(1-\frac{\sqrt{\mu\alpha}}{4}\right)
\end{equation*}
By choice of $\alpha$ as in \eqref{eq:para} and simple calculation we obtain $N = \widetilde{O}(1/\epsilon)$ when $\epsilon$ is small. Now we have
\begin{equation*}
    \|y_{I+1}-y_I^*\|^2 = \|y_I^{N}-y_I^*\|^2 \leq \frac{\mu+l_{g,1}}{\mu}\|y_I-y_I^*\|^2 + \frac{\epsilon^2}{16L_0^2} \leq \frac{3\epsilon^2}{16L_0^2},
\end{equation*}
which yields 
\begin{equation*}
    \|y_{I+1}-y_{I+1}^*\| 
    \leq \|y_{I+1}-y_I^*\| + \|y_I^*-y_{I+1}^*\|
    \leq \frac{\sqrt{3}\epsilon}{4L_0} + \frac{\eta l_{g,1}}{\mu} \leq \frac{\epsilon}{2L_0},
\end{equation*}
where we choose $1-\beta$ to be small (see \eqref{eq:thm-beta} for details) such that $\eta$ is small enough to make above inequality holds.
% $\|y_{I+1}-y_{I+1}^*\|\leq \epsilon/2L_0$. 
Repeating the same process yields the result.
\end{proof}

\subsection{Proof of \Cref{lem:averaging}}
\begin{lemma}[Averaging, Restatement of \Cref{lem:averaging}] \label{lm:averaging}
Under \Cref{ass:relax-smooth},~\ref{ass:f-and-g},~\ref{ass:noise},~\ref{ass:individual-noise} and event $\gE_{\init}\cap\gE_y^1$ (Option I) or $\gE_{\init}\cap\gE_y^2$ (Option II), we further set $\tau=\sqrt{\mu\alpha}$ in the averaging step (line 21 of \Cref{alg:bilevel}). Then for any $t\geq 0$ we have 
\begin{equation*}
    \|\hat{y}_t-y_t^*\| \leq \frac{2\epsilon}{L_0}
    \quad\text{and}\quad
    \|\hat{y}_{t+1}-\hat{y}_t\| \leq \frac{\mu\epsilon^2}{24L_0^2\sigma_{g,1}} =: \vartheta.
\end{equation*}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:averaging}]
We will first show the following result by induction, i.e., for any $t\geq0$, the averaged sequence $\{\hat{y}_t\}$ satisfies
\begin{equation} \label{eq:hat-y-induction}
    \begin{aligned}
        \|\hat{y}_t-y_t^*\| \leq \frac{(1-\tau)\eta l_{g,1}}{\tau\mu} + \frac{\epsilon}{L_0}.
    \end{aligned}
\end{equation}
For $t=0$, by \Cref{eq:warm-start} we have
\begin{equation*}
    \|\hat{y}_0-y_0^*\| = \|y_{T_0}^{\init}-y_0^*\| \leq \sqrt{\frac{\mu}{8(\mu+l_{g,1})}}\frac{\epsilon}{L_0} \leq \frac{\epsilon}{L_0},
\end{equation*}
thus the base case holds. Now suppose \eqref{eq:hat-y-induction} holds for some $t\geq 0$, then for time step $t+1$ we have
\begin{equation*}
    \begin{aligned}
        \|\hat{y}_{t+1} - y_{t+1}^*\|
        &= \|(1-\tau)(\hat{y}_t-y_{t+1}^*) + \tau(y_{t+1}-y_{t+1}^*)\| \\
        &= \|(1-\tau)(\hat{y}_t-y_t^*) + (1-\tau)(y_t^*-y_{t+1}^*) + \tau(y_{t+1}-y_{t+1}^*)\| \\
        &\leq (1-\tau)\|\hat{y}_t-y_t^*\| + (1-\tau)\|y_t^*-y_{t+1}^*\| + \tau\|y_{t+1}-y_{t+1}^*\| \\
        &\leq (1-\tau)\left(\frac{(1-\tau)\eta l_{g,1}}{\tau\mu} + \frac{\epsilon}{L_0}\right) + \frac{(1-\tau)\eta l_{g,1}}{\mu} + \frac{\tau\epsilon}{L_0} \\
        &\leq \frac{(1-\tau)\eta l_{g,1}}{\tau\mu} + \frac{\epsilon}{L_0},
    \end{aligned}
\end{equation*}
where we use induction hypothesis in the second inequality. Therefore, we have that \eqref{eq:hat-y-induction} holds for any $t\geq0$.
Also, as a consequence, for any $t\geq0$ we have
\begin{equation*}
    \begin{aligned}
        \|\hat{y}_{t+1} - \hat{y}_t\|
        &= \|\tau(y_{t+1}-\hat{y}_t)\| \\
        &\leq \tau\|y_{t+1}-y_{t+1}^*\| + \tau\|y_{t+1}^*-y_t^*\| + \tau\|y_t^*-\hat{y}_t\| \\
        &\leq \tau\left(\frac{\epsilon}{L_0} + \frac{\eta l_{g,1}}{\mu} + \frac{(1-\tau)\eta l_{g,1}}{\tau\mu} + \frac{\epsilon}{L_0}\right) \\
        &= \tau\left(\frac{\eta l_{g,1}}{\tau\mu} + \frac{2\epsilon}{L_0}\right).
    \end{aligned}
\end{equation*}
Now we plug in the definition of $\alpha,\beta,\tau,\eta$ as in \eqref{eq:para} to obtain 
\begin{equation*}
    \begin{aligned}
        \|\hat{y}_t-y_t^*\| 
        \leq \frac{(1-\tau)\eta l_{g,1}}{\tau\mu} + \frac{\epsilon}{L_0} 
        = \frac{\sigma_{g,1}}{\mu}\sqrt{1-\beta} + \frac{\epsilon}{L_0} \leq \frac{2\epsilon}{L_0}
    \end{aligned}
\end{equation*}
and 
\begin{equation*}
    \begin{aligned}
        \|\hat{y}_{t+1}-\hat{y}_t\| 
        \leq \tau\left(\frac{\eta l_{g,1}}{\tau\mu} + \frac{2\epsilon}{L_0}\right) \leq \frac{\mu\epsilon^2}{24L_0^2\sigma_{g,1}}.
    \end{aligned}
\end{equation*}
\end{proof}



\subsection{Proof of \Cref{lem:uppererror}}
\begin{lemma}[Restatement of \Cref{lem:uppererror}] \label{lm:x-momentum-recursion}
Under \Cref{ass:relax-smooth},~\ref{ass:f-and-g},~\ref{ass:noise},~\ref{ass:individual-noise} and event $\gE_{\init}\cap\gE_y^1$ (Option I) or $\gE_{\init}\cap\gE_y^2$ (Option II), define $\epsilon_t = m_t-\E_t[\gdf(x_t,\hat{y}_t;\Bar{\xi}_t)]$, then we have the following averaged cumulative error bound:
\begin{equation*}
    \begin{aligned}
        \frac{1}{T}\sum_{t=0}^{T-1}\E\|\epsilon_t\|
        &\leq \frac{\Bar{\sigma}}{T(1-\beta)} + \sqrt{1-\beta}\Bar{\sigma} + \frac{\Bar{L}_0}{\sqrt{1-\beta}}\sqrt{\frac{2(\eta^2+\vartheta^2)}{S}} + \Bar{L}_1\sqrt{\frac{2(\eta^2+\vartheta^2)}{S(1-\beta)}}\frac{1}{T}\sum_{t=0}^{T-1}\E\|\gdphi(x_t)\|.
    \end{aligned}
\end{equation*}
\end{lemma}

\begin{proof}[Proof of \Cref{lm:x-momentum-recursion}]
Define $\epsilon_t = m_t-\E_t[\gdf(x_t,\hat{y}_t;\Bar{\xi}_t)]$, also define $\tilde{\epsilon}_t$ and $\hat{\epsilon}_t$ as
\begin{equation*}
    \begin{aligned}
        \Tilde{\epsilon}_t &= \gdf(x_t,\hat{y}_t;\Bar{\xi}_t) - \E_t[\gdf(x_t,\hat{y}_t;\Bar{\xi}_t)], \\
        \hat{\epsilon}_t &= \gdf(x_t,\hat{y}_t;\Bar{\xi}_t) - \gdf(x_{t-1},\hat{y}_{t-1};\Bar{\xi}_t) - \E_t[\gdf(x_t,\hat{y}_t;\Bar{\xi}_t)] + \E_t[\gdf(x_{t-1},\hat{y}_{t-1};\Bar{\xi}_t)]. \\
    \end{aligned}
\end{equation*}
By definition of $\epsilon_t$, $\tilde{\epsilon}_t$ and $\hat{\epsilon}_t$, we have the following recursion for any $t\geq 0$:
\begin{equation} \label{eq:momentum-recursion}
    \epsilon_{t+1} = \beta\epsilon_t + (1-\beta)\hat{\epsilon}_{t+1} + \beta\Tilde{\epsilon}_{t+1}.
\end{equation}
Then we apply \eqref{eq:momentum-recursion} recursively to obtain
\begin{equation*}
    \epsilon_t = \beta^t\epsilon_0 + \beta\sum_{i=1}^{t}\beta^{t-i}\Tilde{\epsilon}_i + (1-\beta)\sum_{i=1}^{t}\beta^{t-i}\hat{\epsilon}_i,
\end{equation*}
which by triangle inequality and total expectation gives
\begin{equation} \label{eq:momentum-recursion-1}
    \E\|\epsilon_t\| = \beta^t\underbrace{\E\|\epsilon_0\|}_{Err_1} + (1-\beta)\underbrace{\E\left\|\sum_{i=1}^{t}\beta^{t-i}\hat{\epsilon}_i\right\|}_{Err_2} + \beta\underbrace{\E\left\|\sum_{i=1}^{t}\beta^{t-i}\Tilde{\epsilon}_i\right\|}_{Err_3}.
\end{equation}
\paragraph{Bounding $Err_1$.}
By definition of $\epsilon_0$ and \Cref{lm:hyper-var}, along with Jensen's inequality, we have
\begin{equation} \label{eq:Err-1}
    \E\|\epsilon_0\| \leq \sqrt{\E\|\epsilon_0\|^2} \leq \Bar{\sigma}.
\end{equation}
\paragraph{Bounding $Err_2$.}
We apply \Cref{lm:hyper-var} and follow the similar procedure as in \cite[Lemma D.9]{hao2024bilevel} to obtain
\begin{equation} \label{eq:Err-2}
    \E\left\|\sum_{i=1}^{t}\beta^{t-i}\tilde{\epsilon}_i\right\| 
    \leq \sqrt{\E\left\|\sum_{i=1}^{t}\beta^{t-i}\tilde{\epsilon}_i\right\|^2}
    \leq \sqrt{\sum_{i=1}^{t}\beta^{2(t-i)}\E\|\tilde{\epsilon}_i\|^2}
    \leq \frac{\Bar{\sigma}}{\sqrt{1-\beta}},
\end{equation}
where we use Jensen's inequality for the first step.
\paragraph{Bounding $Err_3$.}
We will first use induction to show that for $0\leq i\leq t+1$, the following inequality holds:
\begin{small}
\begin{equation} \label{eq:induction-error}
    \begin{aligned}
        \E\left[\left\|\sum_{j=1}^{t}\beta^{t-j}\hat{\epsilon}_j\right\|\right] 
        \leq \sqrt{\frac{2(\eta^2+\vartheta^2)}{S}}\Bar{L}_1\sum_{j=t+1-i}^{t}\beta^{t-j}\E\|\gdphi(x_j)\| + \E\left[\sqrt{\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i}\beta^{2j-2} + \left\|\sum_{j=1}^{t-i}\beta^{t-j}\hat{\epsilon}_j\right\|^2}\right].
    \end{aligned}
\end{equation}
\end{small}%
Then it's easy to check that by setting $i=t+1$ we can obtain the bound. When $i=0$, \eqref{eq:induction-error} holds obviously since
\begin{small}
\begin{equation*}
    \E\left[\left\|\sum_{j=1}^{t}\beta^{t-j}\hat{\epsilon}_j\right\|\right] 
    \leq \E\left[\sqrt{\left\|\sum_{j=1}^{t}\beta^{t-j}\hat{\epsilon}_j\right\|^2}\right]
    = \E\left[\left\|\sum_{j=1}^{t}\beta^{t-j}\hat{\epsilon}_j\right\|\right].
\end{equation*}
\end{small}%
Hence the base case stands. Now suppose \eqref{eq:induction-error} holds for some $i\geq 0$, and we aim to show that \eqref{eq:induction-error} holds for $i+1$. In fact, we have
\begin{small}
% \begin{equation*}
    \begin{align}
        &\E\left[\sqrt{\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i}\beta^{2j-2} + \left\|\sum_{j=1}^{t-i}\beta^{t-j}\hat{\epsilon}_j\right\|^2}\right] \\
        &= \E_{\gF_{t-i-1}}\left[\E_{t-i-1}\left[\sqrt{\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i}\beta^{2j-2} + \left\|\sum_{j=1}^{t-i}\beta^{t-j}\hat{\epsilon}_j\right\|^2}\right]\right] \label{eq:line-1} \\
        &\leq \E_{\gF_{t-i-1}}\left[\E_{t-i-1}\sqrt{\left[\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i}\beta^{2j-2} + \left\|\sum_{j=1}^{t-i}\beta^{t-j}\hat{\epsilon}_j\right\|^2\right]}\right] \label{eq:line-2} \\
        &= \E_{\gF_{t-i-1}}\left[\E_{t-i-1}\sqrt{\left[\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i}\beta^{2j-2} + \beta^{2i}\|\hat{\epsilon}_{t-i}\|^2 + \left\|\sum_{j=1}^{t-i-1}\beta^{t-j}\hat{\epsilon}_j\right\|^2\right]}\right] \label{eq:line-3} \\
        &\leq \E_{\gF_{t-i-1}}\left[\E_{t-i-1}\sqrt{\left[\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i}\beta^{2j-2} + \frac{\beta^{2i}}{S}2(\Bar{L}_0^2+\Bar{L}_1^2\|\gdphi(x_{t-i})\|^2)(\eta^2+\vartheta^2) + \left\|\sum_{j=1}^{t-i-1}\beta^{t-j}\hat{\epsilon}_j\right\|^2\right]}\right] \label{eq:line-4} \\
        &= \E_{\gF_{t-i-1}}\left[\sqrt{\frac{2\beta^{2i}}{S}\Bar{L}_1^2(\eta^2+\vartheta^2)\|\gdphi(x_{t-i})\|^2+\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i+1}\beta^{2j-2}+\left\|\sum_{j=1}^{t-i-1}\beta^{t-j}\hat{\epsilon}_j\right\|^2}\right] \label{eq:line-5} \\
        &\leq \E_{\gF_{t-i-1}}\left[\sqrt{\frac{2(\eta^2+\vartheta^2)}{S}}\beta^{i}\Bar{L}_1\|\gdphi(x_{t-i})\|+\sqrt{\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{j=1}^{i+1}\beta^{2j-2}+\left\|\sum_{j=1}^{t-i-1}\beta^{t-j}\hat{\epsilon}_j\right\|^2}\right], \label{eq:line-6}
    \end{align}
% \end{equation*}
\end{small}%
where \eqref{eq:line-1} follows by law of total expectation, \eqref{eq:line-2} follows by Jensen's inequality, \eqref{eq:line-3} uses the fact that $\hat{\epsilon}_j$ for $j<t-i$ are $\gF_{t-i-1}$-measurable, and are uncorrelated with $\hat{\epsilon}_{t-i}$; for \eqref{eq:line-4} we use \Cref{lm:hyper-estimator} and~\ref{lm:averaging} to derive
\begin{equation*}
    \begin{aligned}
        \E_{t-i-1}[\|\hat{\epsilon}_{t-i}\|^2]
        &= \E_{t-i-1}\left[\|\gdf(x_{t-i},\hat{y}_{t-i};\Bar{\xi}_{t-i}) - \gdf(x_{t-i-1},\hat{y}_{t-i-1};\Bar{\xi}_{t-i}) \right.\\
        &\quad\left.- \E_{t-i}[\gdf(x_{t-i},\hat{y}_{t-i};\Bar{\xi}_{t-i})] + \E_{t-i}[\gdf(x_{t-i-1},\hat{y}_{t-i-1};\Bar{\xi}_{t-i})]\|^2\right] \\
        &\leq \E_{t-i-1}\left[\|\gdf(x_{t-i},\hat{y}_{t-i};\Bar{\xi}_{t-i}) - \gdf(x_{t-i-1},\hat{y}_{t-i-1};\Bar{\xi}_{t-i})\|^2\right] \\
        &\leq 2\E_{t-i-1}\left[\|\gdf(x_{t-i},\hat{y}_{t-i};\Bar{\xi}_{t-i}) - \gdf(x_{t-i},\hat{y}_{t-i-1};\Bar{\xi}_{t-i})\|^2\right] \\
        &\quad+ 2\E_{t-i-1}\left[\|\gdf(x_{t-i},\hat{y}_{t-i-1};\Bar{\xi}_{t-i}) - \gdf(x_{t-i-1},\hat{y}_{t-i-1};\Bar{\xi}_{t-i})\|^2\right] \\
        &\leq \frac{2}{S}(\Bar{L}_0^2+\Bar{L}_1^2\|\gdphi(x_{t-i})\|^2)(\|\hat{y}_{t-i}-\hat{y}_{t-i-1}\|^2 + \|x_{t-i}-x_{t-i-1}\|^2) \\
        &= \frac{2}{S}(\Bar{L}_0^2+\Bar{L}_1^2\|\gdphi(x_{t-i})\|^2)(\eta^2+\vartheta^2).
    \end{aligned}
\end{equation*}
And \eqref{eq:line-5} follows from the fact that $x_{t-i}$ is $\gF_{t-i-1}$-measurable, \eqref{eq:line-6} uses $\sqrt{a+b}\leq \sqrt{a}+\sqrt{b}$ for $a,b\geq0$. Hence the induction proof is completed. We set $i=t+1$ to obtain 
\begin{equation} \label{eq:Err-3}
    \begin{aligned}
        \E\left[\left\|\sum_{i=1}^{t}\beta^{t-i}\hat{\epsilon}_i\right\|\right] 
        &\leq \sqrt{\frac{2(\eta^2+\vartheta^2)}{S}}\Bar{L}_1\sum_{i=0}^{t}\beta^{t-i}\E\|\gdphi(x_i)\| + \sqrt{\frac{2(\eta^2+\vartheta^2)\Bar{L}_0^2}{S}\sum_{i=0}^{t}\beta^{2i}} \\
        &\leq \sqrt{\frac{2(\eta^2+\vartheta^2)}{S}}\Bar{L}_1\sum_{i=0}^{t}\beta^{t-i}\E\|\gdphi(x_i)\| + \frac{\Bar{L}_0}{\sqrt{1-\beta}}\sqrt{\frac{2(\eta^2+\vartheta^2)}{S}}.
    \end{aligned}
\end{equation}
\paragraph{Final Bound.}
Combining \eqref{eq:Err-1}, \eqref{eq:Err-2} and \eqref{eq:Err-3} yields
\begin{equation*}
    \begin{aligned}
        \E\|\epsilon_t\|
        &\leq \beta^t\Bar{\sigma} + \sqrt{1-\beta}\Bar{\sigma} + \frac{\Bar{L}_0}{\sqrt{1-\beta}}\sqrt{\frac{2(\eta^2+\vartheta^2)}{S}} + \sqrt{\frac{2(\eta^2+\vartheta^2)}{S}}\Bar{L}_1\sum_{i=0}^{t}\beta^{t-i}\E\|\gdphi(x_i)\|.
    \end{aligned}
\end{equation*}
Taking summation and dividing $1/T$ on both sides gives the final result
\begin{equation*}
    \begin{aligned}
        \frac{1}{T}\sum_{t=0}^{T-1}\E\|\epsilon_t\|
        &\leq \frac{\Bar{\sigma}}{T(1-\beta)} + \sqrt{1-\beta}\Bar{\sigma} + \frac{\Bar{L}_0}{\sqrt{1-\beta}}\sqrt{\frac{2(\eta^2+\vartheta^2)}{S}} + \Bar{L}_1\sqrt{\frac{2(\eta^2+\vartheta^2)}{S(1-\beta)}}\frac{1}{T}\sum_{t=0}^{T-1}\E\|\gdphi(x_t)\|.
    \end{aligned}
\end{equation*}
\end{proof}
